Robust Data Pruning under Label Noise via Maximizing Re-labeling Accuracy

Data pruning, which aims to downsize a large training set into a small informative subset, is crucial for reducing the enormous computational costs of modern deep learning. Though large-scale data collections invariably contain annotation noise and numerous robust learning methods have been developed, data pruning for the noise-robust learning scenario has received little attention. With state-of-the-art Re-labeling methods that self-correct erroneous labels while training, it is challenging to identify which subset induces the most accurate re-labeling of erroneous labels in the entire training set. In this paper, we formalize the problem of data pruning with re-labeling. We first show that the likelihood of a training example being correctly re-labeled is proportional to the prediction confidence of its neighborhood in the subset. Therefore, we propose a novel data pruning algorithm, Prune4Rel, that finds a subset maximizing the total neighborhood confidence of all training examples, thereby maximizing the re-labeling accuracy and generalization performance. Extensive experiments on four real and one synthetic noisy datasets show that \algname{} outperforms the baselines with Re-labeling models by up to 9.1% as well as those with a standard model by up to 21.6%.

==> 8-rebuttal.tex <==
\appendix

\begin{center}
\Large Robust Data Pruning under Label Noise via \\ Maximizing Re-labeling Accuracy \\
\vspace{0.1cm}
\Large(Global Response for Rebuttal)%\bigskip
\end{center}


\setcounter{figure}{2}

\begin{wrapfigure}{R}{0.5\linewidth}
%\begin{figure}[t!]
\begin{center}
\includegraphics[width=7cm]{figures/figure_rebuttal_clothing1m.pdf}
\end{center}
\vspace{-0.3cm}
\caption{Test accuracy of DivideMix fine-tuned on each selected subset of Clothing-1M.}
\vspace{-0.5cm}
%\end{figure}
\label{fig:rebuttal}
\end{wrapfigure}

==> tables/confidence_metrics_noisy_ratio.tex <==
\begin{table*}[!t]
\noindent
\small
%\caption{Funny Table Examples.} 
\parbox{.4\textwidth}{%
\parbox{5.0cm}{
\vspace{0.4cm}
\caption{Effect of the confidence metrics on \algname{} with SOP+.}
\vspace{0.1cm}
\label{table:effect_of_meta_input}
}
\scriptsize
\begin{tabular}{c|c|c c c c}\toprule
\multirow{2}{*}{\makecell[c]{\!\!\!Dataset\!\!\!}}& \multirow{2}{*}{\makecell[c]{\!\!\!Conf. Metric\!\!\!}} & \multicolumn{4}{c}{Selection Ratio} \\
& & 0.2&0.4&0.6&0.8\\ \midrule
\multirow{2}{*}{\makecell[c]{\!\!\!CIFAR-10N\\(Worst)\!\!\!}}& MaxProb & 83.4&89.3&91.5&92.5\\
& DiffProb &83.1&89.2&91.6&92.5\\ \midrule
\multirow{2}{*}{\makecell[c]{\!\!\!CIFAR-100N\!\!\!}}& MaxProb & 49.0&59.1&64.1&65.7\\
& DiffProb &48.6&59.9&64.0&66.0\\ \bottomrule
\end{tabular}
%\begin{tabular}{c|c c c c}\toprule
%Dataset & \multicolumn{4}{c}{CIFAR-10N (Worst)} \\ 
%Select Ratio & 0.2 & 0.4 & 0.6 & 0.8\\ \midrule
%MaxConf & 0.2 & 0.4 & 0.6 & 0.8\\
%MaxMargin & 0.2 & 0.4 & 0.6 & 0.8\\ \midrule
%Dataset & \multicolumn{4}{c}{CIFAR-100N} \\ 
%MaxConf & 0.2 & 0.4 & 0.6 & 0.8\\
%MaxMargin & 0.2 & 0.4 & 0.6 & 0.8\\ \bottomrule
%\end{tabular}
}%
\parbox{.6\textwidth}{%
\parbox{8.0cm}{
\vspace{0.4cm}
\caption{Ratio of noisy examples in the selected subset.}
\vspace{0.1cm}
\label{table:effect_of_meta_input}
}
\scriptsize
\begin{tabular}{c|c c c c|c c c c}\toprule
Dataset & \multicolumn{4}{c|}{\underline{CIFAR-10N (Worst)}} & \multicolumn{4}{c}{\underline{CIFAR-100N}} \\
Sel. Ratio & 0.2 & 0.4 & 0.6 & 0.8 & 0.2 & 0.4 & 0.6 & 0.8 \\ \midrule
SmallL & 0.8 & 3.6 & 11.5 & 26.2 & 3.5 & 8.7 & 16.3 & 27.4 \\
Margin & 54.6 & 52.1 & 48.5 & 44.6 & 61.5 & 56.8 & 51.6 & 46.2 \\
kCenter & 40.0 & 41.1 & 41.6 & 42.1 & 37.5 & 38.7 & 39.9 & 40.4 \\
Forget & 37.7 & 38.8 & 39.2 & 40.2 & 37.9 & 34.6 & 33.0 & 36.8 \\
GraNd & 91.5 & 79.4 & 64.2 & 50.1 & 93.9 & 57.3 & 61.2 & 49.3 \\
\textbf{\algname{}} & 38.7 & 42.7 & 43.5 & 46.5 & 28.3 & 29.1 & 33.3 & 37.2 \\ \bottomrule
\end{tabular}
}%
\vspace*{-0.3cm}
\end{table*}




==> tables/experiment_detail_2.tex <==
\def\arraystretch{1.15}% make the row margin compact
\begin{table*}[t!]
% \small
% \tiny
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\begin{tabular}{lc|c|c|c|c}
\midrule
\multicolumn{2}{l|}{\multirow{1}{*}{}} & \multirow{1}{*}{\textbf{CIFAR10N}} & \multirow{1}{*}{\textbf{CIFAR100N}} & \multirow{1}{*}{\textbf{WebVision}} & \multirow{1}{*}{\textbf{Clothing1M}} \\
\midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{SOP+}}} & \textbf{lr for $u_{i}$, $v_{i}$} & $\alpha_{u}$=10, $\alpha_{v}$=100 & $\alpha_{u}$=1, $\alpha_{v}$=100 & $\alpha_{u}$=0.1, $\alpha_{v}$=1 & \multicolumn{1}{l}{} \\
\multicolumn{1}{c|}{} & \textbf{wd for $u_{i}$, $v_{i}$} & 0 & 0 & 0 & \multicolumn{1}{l}{} \\
\multicolumn{1}{c|}{} & \textbf{init. std for $u_{i}$, $v_{i}$} & $10^{-8}$ & $10^{-8}$ & $10^{-8}$ & \multicolumn{1}{l}{} \\
\multicolumn{1}{c|}{} & \textbf{$\lambda_{C}$} & 0.9 & 0.9 & 0 & \multicolumn{1}{l}{} \\
\multicolumn{1}{c|}{} & \textbf{$\lambda_{B}$} & 0.1 & 0.1 & 0 & \multicolumn{1}{l}{} \\
\midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\textbf{DivideMix}}} & \textbf{$\lambda_{U}$} & 1 & 1 & \multicolumn{1}{l|}{} & 0 \\
\multicolumn{1}{c|}{} & \textbf{$\tau$} & 0.5 & 0.5 & \multicolumn{1}{l|}{} & 0.5 \\
\multicolumn{1}{c|}{} & \textbf{T} & 0.5 & 0.5 & \multicolumn{1}{l|}{} & 0.5 \\
\multicolumn{1}{c|}{} & \textbf{$\alpha$} & 4 & 4 & \multicolumn{1}{l|}{} & 0.5 \\
\multicolumn{1}{c|}{} & \textbf{M} & 2 & 2 & \multicolumn{1}{l|}{} & 2 \\
\midrule
\multicolumn{1}{l|}{\multirow{9}{*}{}} & \textbf{architecture} & PreAct PresNet18 & PreAct PresNet18 & InceptionResNetV2 & \begin{tabular}[c]{@{}c@{}}ResNet-50 \\ (pretrained)\end{tabular} \\
\multicolumn{1}{l|}{} & \textbf{batch size} & 128 & 128 & 32 & 32 \\
\multicolumn{1}{l|}{} & \textbf{learning rate(lr)} & 0.02 & 0.02 & 0.02 & 0.002 \\
\multicolumn{1}{l|}{} & \textbf{lr decay} & Cosine Annealing & Cosine Annealing & MultiStep-50th & MultiStep-5th \\
\multicolumn{1}{l|}{} & \textbf{weight decay} & $5 \times 10^{-4}$ & $5 \times 10^{-4}$ & $5 \times 10^{-4}$ & 0.001 \\
\multicolumn{1}{l|}{} & \textbf{training epoch} & 300 & 300 & 100 & 10 \\
\multicolumn{1}{l|}{} & \textbf{warm-up epoch} & 10 & 30 & 10 & 0 (forget 5) \\
\multicolumn{1}{l|}{} & \textbf{training examples} & 50,000 & 50,000 & 66,000 & 1,000,000 \\
\multicolumn{1}{l|}{} & \textbf{optimizer} & \begin{tabular}[c]{@{}c@{}}SGD\\ (momentum 0.9)\end{tabular} & \begin{tabular}[c]{@{}c@{}}SGD\\ (momentum 0.9)\end{tabular} & \begin{tabular}[c]{@{}c@{}}SGD\\ (momentum 0.9)\end{tabular} & \begin{tabular}[c]{@{}c@{}}SGD\\ (momentum 0.9)\end{tabular} \\
\midrule
\end{tabular}
\caption{Hyper-parameters for SOP+ and DivideMix on CIFAR-10N/100N, Clothing-1M and Webvision datasets.}
\label{table:experiment_detail}
\end{table*}

==> tables/perf_ImageNet.tex <==
\begin{table*}[!t]
\noindent
\small
\vspace*{-0.0cm}
\caption{Data pruning performance on ImageNet with 20$\%$ label noise.} 
\centering
\scriptsize
\begin{tabular}{c|c|c c c c}\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{ReLabel\\Model}\hspace{-0.10cm}}&\multirow{2}{*}{\makecell[c]{Selection\\Methods}}& \multicolumn{4}{c}{\underline{ImageNet-1K (Syn, $\approx\!20\%$)}} \\
& & 0.05 & 0.1 & 0.2 & 0.4 \\ \midrule
\multirow{4}{*}{SOP+}&Uniform & 27.8 & 42.5 & 52.7 & 59.2 \\
&SmallL & 22.8 & 31.4 & 42.7 & 54.4\\
&Forget& 4.1 & 8.3 & 50.6 & 57.2\\
&\textbf{$\text{\tblalgname{}}_B$}& \textbf{30.2} & \textbf{44.3} & \textbf{53.5} & \textbf{60.0}\\ \bottomrule
\end{tabular}
\vspace*{-0.2cm}
\label{table:results_imagenet}
\end{table*}

==> tables/perf_tbl.tex <==
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.1}% make the row margin compact
\begin{table*}[t!]
% \small
% \tiny
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Performance comparison of sample selection baselines and \algname{} on CIFAR-10N and CIFAR-100N. The best results are in bold and the second bests are underlined.}
\vspace*{0.2cm}
% \resizebox{1.0\columnwidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}c|c|cccc|cccc|ccccc@{}}
\toprule
\multirow{3}{*}{\hspace{-0.0cm}\makecell[c]{ReLabel\\Models}\hspace{-0.10cm}}&\multirow{3}{*}{\makecell[c]{Pruning\\Methods}}& \multicolumn{8}{c|}{{\underline{CIFAR-10N}}} 
& \multicolumn{4}{c}{{\underline{CIFAR-100N}}}\\%\cline{3-14} 
% \addlinespace[0.6ex]
% \multicolumn{1}{c|}{\hspace{-0.20cm}\textbf{ReLabel}\hspace{-0.20cm}}
% \multicolumn{1}{c|}{\hspace{-0.10cm}\textbf{Pruning}\hspace{-0.20cm}} 
%\addlinespace[0.4ex]
& & \multicolumn{4}{c|}{{Random}} & \multicolumn{4}{c|}{{Worst}} & \multicolumn{4}{c}{{Noisy}} \\
%\addlinespace[-0.2ex]
%\multicolumn{1}{c|}{\hspace{-0.20cm}\textbf{Method}\hspace{-0.20cm}} 
%& \multicolumn{1}{c|}{\hspace{-0.10cm}\textbf{Method}\hspace{-0.20cm}} 
& & \multicolumn{1}{c}{\hspace{-0.20cm}{0.2}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.4}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.6}}
& \multicolumn{1}{c|}{\hspace{-0.20cm}{0.8}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.2}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.4}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.6}}
& \multicolumn{1}{c|}{\hspace{-0.20cm}{0.8}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.2}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.4}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.6}}
& \multicolumn{1}{c}{\hspace{-0.20cm}{0.8}}
\\ \midrule
% # Standard ###############################################################
\multirow{3}{*}{\hspace{-0.0cm}{Standard}\hspace{-0.10cm}}                           
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Uniform\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.5}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.9}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{83.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.6}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.4}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{00}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
% \midrule
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}SmallL\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.1}\scalebox{0.75}{$\pm$4.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.0}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{70.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{80.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.1}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
%\midrule
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Forget\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.1}\scalebox{0.75}{$\pm$4.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.0}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{70.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{80.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.1}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
\midrule
% # DivideMix ###############################################################
\multirow{8}{*}{\hspace{-0.0cm}{DivMix}\hspace{-0.10cm}} 
\begin{comment}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Full\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$0.4}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
\\
\end{comment}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Uniform\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{87.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.9}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{83.2}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{88.5}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.4}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{30.5}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.3}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{57.5}\scalebox{0.75}{$\pm$1.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{58.6}\scalebox{0.75}{$\pm$0.9}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}SmallL\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.1}\scalebox{0.75}{$\pm$4.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.0}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{70.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{80.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.1}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{33.3}\scalebox{0.75}{$\pm$3.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{47.4}\scalebox{0.75}{$\pm$1.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{59.4}\scalebox{0.75}{$\pm$0.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{62.0}\scalebox{0.75}{$\pm$1.2}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Margin\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{68.5}\scalebox{0.75}{$\pm$2.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.5}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.2}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.3}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{75.1}\scalebox{0.75}{$\pm$0.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{85.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.2}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{17.1}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{30.8}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{46.3}\scalebox{0.75}{$\pm$2.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.2}\scalebox{0.75}{$\pm$1.3}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}kCenter\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.4}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{93.0}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.4}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{95.1}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.7}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.4}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.6}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{38.0}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{50.0}\scalebox{0.75}{$\pm$1.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{59.7}\scalebox{0.75}{$\pm$1.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.0}\scalebox{0.75}{$\pm$0.9}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Forget\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{85.2}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{93.0}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{94.5}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{95.1}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{78.3}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.4}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.0}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{26.4}\scalebox{0.75}{$\pm$1.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{54.3}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.1}\scalebox{0.75}{$\pm$1.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{66.6}\scalebox{0.75}{$\pm$1.1}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}GraNd\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{21.8}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{60.9}\scalebox{0.75}{$\pm$4.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.5}\scalebox{0.75}{$\pm$1.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{18.5}\scalebox{0.75}{$\pm$1.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{25.5}\scalebox{0.75}{$\pm$0.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{49.3}\scalebox{0.75}{$\pm$0.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{88.0}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{15.5}\scalebox{0.75}{$\pm$1.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{26.0}\scalebox{0.75}{$\pm$1.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{44.7}\scalebox{0.75}{$\pm$1.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{60.4}\scalebox{0.75}{$\pm$1.6}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{\algname{}}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{87.9}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.5}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{94.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{95.1}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{83.4}}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.5}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{$\text{\algname{}}_B$}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{93.0}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{{19.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{83.6}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.9}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\ \addlinespace[0.1ex]\cline{2-14}\addlinespace[0.1ex]
% \midrule
&\multicolumn{1}{c|}{\hspace{-0.0cm}$\%$ \textit{Improv.}\hspace{-0.10cm}}  
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.7\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}5.7\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}6.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.5\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}9.4\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}-6.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}5.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}21.8\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}-6.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}5.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}21.8\%}\end{tabular}
\\
\midrule
% # DivideMix ###############################################################
% # SOP+ ###############################################################
\multirow{8}{*}{\hspace{-0.0cm}{SOP+}\hspace{-0.30cm}}                             
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Uniform\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{87.5}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.5}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{93.4}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.8}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{81.9}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.5}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{91.8}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{{46.5}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.7}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{60.8}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{64.4}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}SmallL\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{77.6}\scalebox{0.75}{$\pm$2.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{86.2}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.7}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{78.8}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{84.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{89.3}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{48.5}}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{59.8}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{63.9}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{66.1}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Margin\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{52.1}\scalebox{0.75}{$\pm$5.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{79.6}\scalebox{0.75}{$\pm$8.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.6}\scalebox{0.75}{$\pm$3.9}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.1}\scalebox{0.75}{$\pm$1.3}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{45.7}\scalebox{0.75}{$\pm$1.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.8}\scalebox{0.75}{$\pm$0.7}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{84.6}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{92.5}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{20.0}\scalebox{0.75}{$\pm$1.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{34.4}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{50.4}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.3}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}kCenter\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{86.3}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.2}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.1}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{95.3}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{81.9}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{88.0}}\scalebox{0.75}{$\pm$0.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{91.3}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.3}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{44.8}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.9}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{61.6}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{65.2}\scalebox{0.75}{$\pm$0.6}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}Forget\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{82.4}\scalebox{0.75}{$\pm$1.0}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{93.0}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\underline{94.2}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.0}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{71.1}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{87.7}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{90.6}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{92.2}\scalebox{0.75}{$\pm$0.0}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{38.0}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{55.3}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{63.2}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{65.8}\scalebox{0.75}{$\pm$0.4}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}GraNd\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{24.2}\scalebox{0.75}{$\pm$5.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{51.6}\scalebox{0.75}{$\pm$3.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{85.9}\scalebox{0.75}{$\pm$1.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{94.9}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{15.4}\scalebox{0.75}{$\pm$1.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{25.7}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{51.0}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{86.8}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{11.0}\scalebox{0.75}{$\pm$0.1}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{19.0}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{38.7}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{62.1}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{\algname{}}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.2}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{93.0}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{94.4}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{95.1}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{83.4}}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{89.3}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{91.5}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{92.5}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{49.0}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{59.1}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{64.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{65.7}\scalebox{0.75}{$\pm$0.5}\hspace{-0.10cm} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.10cm}\textbf{$\text{\algname{}}_B$}\hspace{-0.20cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{88.6}}\scalebox{0.75}{$\pm$0.5}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{93.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{94.2}}\scalebox{0.75}{$\pm$0.2}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{95.3}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{84.2}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{89.1}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{91.3}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{92.5}}\scalebox{0.75}{$\pm$0.1}\hspace{-0.10cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{52.9}}\scalebox{0.75}{$\pm$0.8}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{60.1}}\scalebox{0.75}{$\pm$0.6}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{64.1}}\scalebox{0.75}{$\pm$0.4}\hspace{-0.20cm} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \hspace{-0.20cm}{\textbf{66.1}}\scalebox{0.75}{$\pm$0.3}\hspace{-0.10cm} }\end{tabular}
\\ \addlinespace[0.1ex]\cline{2-14}\addlinespace[0.1ex]
% \midrule
&\multicolumn{1}{c|}{\hspace{-0.0cm}$\%$ \textit{Improv.}\hspace{-0.10cm}}  
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
%& \begin{tabular}[c]{@{}c@{}}{ - }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}1.3\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}2.8\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}1.5\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.2\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}9.1\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.5\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.3\%}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.20cm}0.0\%}\end{tabular}
\\
\bottomrule
\end{tabular}
% }
\label{tbl:overall_perf}
% \vspace{-0.5cm}
\end{table*}


==> tables/self_correctability.tex <==
\begin{table*}[!t]
\noindent
\small
\vspace*{-0.0cm}
\caption{Data pruning performance on ImageNet with 20$\%$ label noise.} 
\centering
\scriptsize
\begin{tabular}{c|c|c c c}\toprule
\multirow{2}{*}{\hspace{-0.0cm}\makecell[c]{ReLabel\\Model}\hspace{-0.10cm}}&\multirow{2}{*}{\makecell[c]{Selection\\Methods}}& \multicolumn{3}{c}{\underline{CIFAR-10N (Random)}} \\
& & Test Acc. & $\%$ Noisy & $\%$ Self-Correct \\ \midrule
\multirow{3}{*}{SOP+}&kCenter & 86.3 & 19.0 & 75.2 \\
&Forget& 82.4 & 17.0 & 61.7\\
&\textbf{\text{\tblalgname{}}}& {88.2} & {17.0} & \textbf{90.3}\\ \bottomrule
\end{tabular}
\vspace*{-0.2cm}
\label{table:self_correctability}
\end{table*}
